Thinking Inside The Box: Privacy Against Stronger Adversaries

In this thesis, we study extensions of statistical cryptographic primitives. In particular we study leakage-resilient secret sharing, non-malleable extractors, and immunized ideal one-way functions. The thesis is divided into three main chapters. In the first chapter, we show that 2-out-of-2 leakage resilient (and also non-malleable) secret sharing requires randomness sources that are also extractable. This rules out the possibility of using min-entropic sources. In the second, we introduce collision-resistant seeded extractors and show that any seeded extractor can be made collision resistant at a small overhead in seed length. We then use it to give a two-source non-malleable extractor with entropy rate 0.81 in one source and polylogarithmic in the other. The non-malleable extractor lead to the first statistical privacy amplification protocol against memory tampering adversaries. In the final chapter, we study the hardness of the data structure variant of the 3SUM problem which is motivated by a recent construction to immunise random oracles against pre-processing adversaries. We give worst-case data structure hardness for the 3SUM problem matching known barriers in data structures for adaptive adversaries. We also give a slightly stronger lower bound in the case of non-adaptivity. Lastly, we give a novel result in the bit-probe setting.

==> chapters/3sum/multiphase.tex <==
\section{Reduction from Lopsided Set Disjointness}
In this section, we give a reduction from the problem of \emph{Blocked Lopsided Set Disjointness} to the Multiphase $3$SUM problem as defined in Definition \ref{defn:MP3SUM} to obtain the following theorem:

\begin{theorem}
    Any cell probe data structure solving the Multiphase $3$SUM problem using $S = k n^{O(1)}$ memory cells with $t_q = o(\frac{\log(k)}{\log(n)})$ must have $t_u = \omega(\frac{k}{w})$ for the modulo and XOR groups where the size of the group is $k^{1+o(1)}$.
\end{theorem}

\begin{definition}\label{defn:LSD}[Blocked Lopsided Set Disjointness (Blocked LSD)]
    Given two sets $S, T \subseteq [N] \times [B]$ such that Alice is given set $S$, Bob is given set $T$ and is further more such that for all $i \in [N]$, there exists a unique $b_i$ such that $(i, b_i) \in S$, Alice and Bob need to communicate to decide whether $S \cap T = \emptyset$.
\end{definition}
Think of the universe as broken up into $N$ blocks of size $B$ each, and Alice's set is such that for every block, her set contains exactly $1$ element from that block.

Mihai \patrasku\ proved the following communication lower bound for Blocked LSD:
\begin{lemma}[Theorem 4 of \cite{P11}]\label{lemma:lsdLowerBound}
    Fix $\delta > 0$. Any communication protocol for Blocked LSD requires either Alice sending at least $\delta N \log(B)$ bits, or Bob sending at least $NB^{1-O(\delta)}$ bits.
\end{lemma}
For the reduction, we adopt the approach taken in \cite{CGL15} where Alice and Bob will make use of a data structure solving the Multiphase $3$SUM Problem to obtain a communication efficient protocol for Blocked LSD. We will use a technical lemma proved by~\cite{CGL15}:

\begin{lemma}[Lemma 1 of \cite{CGL15}]
    Consider a communication game in which Bob receives a set $B \subseteq [2^w]$ of size $S$ and Alice receives a set $A \subseteq B$ of size $k$. There is a deterministic protocol in which Alice sends $O(k \log(S/k))$ bits, Bob sends $O(kw)$ bits, and after communicating, Bob knows Alice's set $A$.
\end{lemma}

We will want to think of the universe $[N] \times [B]$ as $[k\ell] \times [n / \ell]$ with $k \cdot \ell = N$ and $n / \ell = B$. We then view the universe as having $k$ sets of $\ell$ chunks where each chunk is of size $n / \ell$ for values of $k$, $n$, and $\ell$ to be chosen later. Naturally, any subset $W \subseteq [N] \times [B]$ can be viewed as some collection of $k$ sets $W_i \subseteq [\ell] \times [n / \ell]$. Then letting the collection of sets $X_i$ represent $S$ and $Y_i$ represent $T$, $S \cap T = \emptyset$ if and only if for all $i \in [k]$, $X_i \cap Y_i = \emptyset$.

\begin{proof}
Assuming that there is a pre-processing algorithm for Multiphase $3$SUM using $S$ cells of $w$ bits each such that the update time is $t_u$ and the query time is $t_q$. We build a communication protocol for the Blocked LSD problem in three phases. We first consider this reduction for the cyclic group and show that it essentially holds for the XOR group as well.

We begin by explaining in detail how Alice and Bob should interpret their subsets of $[k\ell] \times [n / \ell]$. Partition $[k\ell]$ into $k$ groups $G_0, \ldots, G_{k-1}$ of $\ell$ elements such that $G_i = \{ i \cdot \ell, i \cdot \ell + 1, \ldots, (i+1) \cdot \ell - 1\}$. Then the universe can be partitioned into $k$ sets $G_i \times [n/\ell]$. It follows that element $(a, r) \in [k\ell] \times [n / \ell]$ corresponds to element $(j, r)$ in the $i^{th}$ subset. We then say that this element is in the $j^{th}$ chunk of the $i^{th}$ set with index $r$. Let $\blocks{X}{k}$ and $\blocks{Y}{k}$ be the collection of Alice's and Bob's subsets of the universe based on the partition. 

\textbf{(Phase 1)} Bob interprets his set $T$ as a collection of $k$ sets $Y_i$ as mentioned above. Then he needs to construct an input set $A_1$ to pre-process. To do this, for every element $(a, r)$ in the universe $[k\ell] \times [n / \ell]$ with $a = i \cdot \ell + j$, we encode it as an integer whose digits can be broken up into $4$ blocks of digits so that conceptually the:
\begin{enumerate}
    \item second digit encodes which chunk of the set the element belongs to using a value in $[\ell]$;
    \item first digit encodes whether the element is present in Bob's set $B$;
    \item third digit encodes which set the element belongs to using a value in $[k]$;
    \item fourth block of digits is such that every digit except for the $j^{th}$ is $0$, and the $j^{th}$ digit is a value $r \in [n / \ell]$ which encodes index of the element in the chunk.
\end{enumerate}

Namely, Bob adds the group element $g$ into $A_1$ such that the $h^{th}$ digit $g[h]$ is given as:
\begin{equation*}
    g[h] = \begin{cases}
         i  &, h = \ell + 2\\
        j &, h = \ell + 1\\
        \indicate{(a, b) \in T} &, h = \ell\\
        r &, h = j - 1\\
        0 &, \text{else}
    \end{cases}
\end{equation*}

Bob now runs the solution for Phase 1 locally with set $A_1$ as input and as a result holds a data structure $D$. Note that during Phase 1, no communication happens between Alice and Bob.

\textbf{(Phase 2)} 
We will want $A_2$ to be a set of elements $g$ whose digits can be broken up into $4$ blocks of digits so that conceptually the:
\begin{enumerate}
    \item first digit is $0$;
    \item second digit is $-j$ for some $j \in [\ell]$;
    \item third digit is some $0$;
    \item fourth block of digits is such that the $j^{th}$ digit is $0$, and can take on any other possible value in $[\frac{n}{\ell}]$ at other digits.
\end{enumerate}

More formally, define $A_2$ to be a set that contains any group element $g$ such that for some $j \in [\ell]$, the $h^{th}$ digit $g[h]$ satisfies:
\begin{equation*}
    g[h] = \begin{cases}
        0 &, h = \ell + 2\\
        2\ell -j &, h = \ell + 1\\
        0 &, h = \ell\\
        0 &, h = j - 1
    \end{cases}
\end{equation*}
Furthermore, any other digit takes on a value in range $[0, \frac{n}{\ell} - 1]$.

For the reduction in the modulo setting, we consider the set of integers in $[k^{1+o(1)}]$. To that end, the encoding works by letting the $3 + \ell$ digits specify a mixed-radix number where most significant digit is in base $k$, the second most in base $2\ell$, the third digit in base $4$, and the remaining digits in base $n / \ell$.

Define $C$ to be Alice's view of $D$ that is initially empty. Alice will then run the update operation with $A_2$ as the input set. Throughout the process, if Alice ever requires a memory cell that does not exist in $C$, Alice will request for the corresponding memory cell from Bob by communicating its index into the data structure using $\log(S) \leq \log(k) + O(\log (n)) \leq \Omega(w)$ bits. Bob then responds with the contents of the memory cell which consists of $w$ bits which Alice then stores into $C$. If the required memory cell is already in $C$, Alice updates the contents of the memory cell locally. The total amount of communication sent by both Alice and Bob is bounded by $t_u \cdot w$.

\textbf{(Phase 3)} Alice now needs to determine whether $X_i \cap Y_i = \emptyset$ for all $i \in [k]$. Recall that for $X_i \subseteq [\ell] \times [\frac{n}{\ell}]$, for each of the chunks $j$, there exists a unique element $b_j \in [\frac{n}{\ell}]$ such that $(j, b_j) \in X_i$.

We construct query element $q_i$ with $\ell + 3$ digits such that the $h^{th}$ digit $q[h]$ satisfies:
\begin{equation*}
    q[h] = \begin{cases}
        i &, h = \ell + 2\\
        0 &, h = \ell + 1\\
        1 &, h = \ell\\
        b_h &, 0 \leq h \leq \ell - 1
    \end{cases}
\end{equation*}
where $(h, b_h) \in X_i$. Alice has $k$ such query values $q_i$ and will run the query algorithm for all of them in parallel. For $t \in [t_q]$, Alice runs the $t^{th}$ step locally. There are at most $k$ cells that Alice needs to complete the step. For any cell that is contained in $C$, Alice is able to obtain the contents of the cell without any communication. Otherwise there are at most $k$ cells that are not in $C$, Alice then communicates $O(\log(S/k)) = O(\log(n))$ bits to Bob to specify the cells that she needs from the data structure. Bob then responds using at most $k \cdot w$ bits. If any of the $k$ queries leads to a YES answer, Alice then outputs NO. Otherwise, Alice outputs YES.

We will show that there exists an $i \in [k]$ such that $X_i \cap Y_i = \emptyset$ if and only if any of the query values $q_i$ leads to a NO answer. We first make the following claim:

\begin{claim}\label{claim:noCarry}
    Let $a_1 \in A_1$ and $a_2 \in A_2$. The second most significant digit of $a_1 + a_2$ is $0$ if and only if $a_1[\ell+1] = j$ and $a_2[\ell+1] = 2\ell-j$ for some $j \in [\ell]$.
\end{claim}

\begin{proof}
    Note that for any possible obtainable pair sum, the third most significant digit's value is at most $2 < 4$, and thus the second most significant digit's value in the sum is only based on the second most significant digit of both operands. Thus it must be the case that $a_1[\ell+1] = j$ and $a_2[\ell+1] = -j$ for some $j \in [\ell]$.
\end{proof}

The above claim implies that Alice obtains a YES answer to query value $q_1$ if and only if there exists some $j \in [\ell]$ for which the three most significant digits if $a_1$ and $a_2$ are given as $i, j, 1$ and $0, -j, 1$ respectively, and furthermore that the $j^{th}$ least significant digit of $a_1$ and of $q_i$ are the same which holds if and only if $X_i \cap Y_i \neq \emptyset$. We can then conclude that the reduction holds.

On the other hand, for the XOR group, Claim \ref{claim:noCarry} also asserts that the only common digit of $a_1$ and of $a_2$ that is both non-zero is the second most significant which means that the group operation behaves exactly the same over the XOR group and the correctness argument holds analogously so long as we write represent $-j$ using the one's complement representation.

Choosing $\ell = \sqrt{t_q \cdot \frac{\log(k)}{\log(n)}}$, we get that $\ell = \omega(t_q)$ and $\ell = o(\frac{\log(k)}{\log(n)})$.

It follows by Lemma \ref{lemma:lsdLowerBound} that Alice has to send $\Omega(k\ell \log(n/\ell)) = \omega (k t_q \log(n))$ bits, or Bob has to send $k \ell (n / \ell)^{3/4} = \omega(k w^2)$ bits. Overall, Alice sends $t_u w + O(k\log(n) t_q)$ and Bob sends $t_u w + O(k w t_q) = t_u w + o(k w^2) $ bits. Therefore we know that $t_u w = \omega(t_q k \log(n)) \implies t_u w = \omega(k) \implies t_u = \omega(k/w)$. 

Lastly, we need to bound the size of sets $A_1$, $A_2$ and the group $G$. By definition, the set $A_1$ is of cardinality $NB = kn$. On the other hand, to bound the cardinality of set $A_2$:
\begin{equation*}
    \ell \left(\frac{n}{\ell} \right)^{\ell - 1} < n^{\ell} = n^{o(\frac{\log k}{\log n})} = k^{o(1)}
\end{equation*}

As for the group size:
\begin{equation*}
    8 k \ell   \left(\frac{n}{\ell} \right)^{\ell} < k n^{\ell} = kn^{o(\frac{\log k}{\log n})} = k^{1+o(1)}
\end{equation*}
\end{proof}

==> chapters/3sum/prelim.tex <==
\section{Preliminaries}
% you should talk about how there's two formally defined versions and we will be dealing with one the two and you should prove the equivalence 
\subsection{$3$SUM-Indexing}
The $3$SUM-Indexing problem was first defined by Demaine and Vadhan in an unpublished manuscript \cite{DV01} and then by Goldstein, Kopelowitz, Lewenstein, and Porat in \cite{GKLP17}. 
\begin{definition}[$3$SUM-Indexing]\label{defn:3sumIndexing}
    Let $(G, +)$ be an finite abelian group. Pre-process two sets of group elements $A_1, A_2 \subseteq G$ each of size $n$ into a data structure $D$ of $S$ memory cells of $w$ bits so that given any query group element $z$, deciding whether there exists $a_1 \in A_1$ and $a_2 \in A_2$ such that $a_1 + a_2 = z$ is done by accessing at most $T$ memory cells.
\end{definition}

Golovnev, Guo, Horel, Park, and Vaikuntanathan in~\cite{GGHPV20} then defined a similar variant of the problem which additionally asserted that the input sets $A_1$ and $A_2$ should be the same.
We first show that the two definitions are essentially equivalent up to a small change in the group. 
i.e. Any solution that solves the~\cite{GGHPV20} variant of $3$SUM-Indexing can also be adapted to solve the variant in Definition~\ref{defn:3sumIndexing}.

\begin{lemma}
    Any pre-processing solution that solves $3$SUM-Indexing as defined in Definition \ref{defn:3sumIndexing} for input sets of size $n$ and universe sizes of $u$ can also be used to solve $3$SUM-Indexing as defined in \cite{GGHPV20}. 
\end{lemma}

\begin{proof}
    For any abelian group $(G', +')$, we define $(G, +)$ to be the group obtained as the direct product of $(\bit, +)$ and $(G', +')$. Then, given any two sets $A_1$ and $A_2$, we construct set $A = \{0\} \times A_1 \cup \{1\} \times A_2$. For any query value $z$, we then form the query as $(1, z)$. In our transformation, the group size and input array length is doubled.

    Assuming that there exists a pair $a_1 \in A_1$ and $a_2 \in A_2$ such that $a_1 + a_2 = z$, then $(0, a_1), (1, a_2)$ is in $A$ and so $(0, a_1) + (1, a_2) = (1, z)$. On the other hand, assuming that no such pairing exists, then no such pairing $(0, a_1), (1, a_2) \in A$ sums to $(1, z)$ as well.
\end{proof}

We also introduce a new variant of the $3$SUM-Indexing problem with updates for data structures which may be of independent interest.

\begin{definition}[Multiphase $3$SUM]\label{defn:MP3SUM}
    The Multiphase $3$SUM problem has three phases. In phase I, we receive a set $A_1$ of $k n$ group elements from some group $(G, +)$ of size $k^{1+o(1)}$ and must pre-process this into a data structure. In phase II, we are then given another set of $A_2$ of $k^{o(1)}$ group elements, and are allowed to make $t_u$ probes to update the data structure. In phase III, we are given a query group element $z$ and have to output whether there exists an element $a_1$ from $A_1$ and $a_2$ from $A_2$ such that $a_1 + a_2 = z$ using at most $t_q$ probes into the data structure.
\end{definition}

==> chapters/ap-publication.tex <==
\begin{refsection}
\nocite{%
  TR04:Arasu,
  nsdi12:Zaharia,
  tods76:Chen,
}

\defbibnote{PubListPrenote}{%
% provide some text, if any, before the list of publications
}
\defbibnote{PubListPostnote}{%
% provide some text, if any, after the list of publications
}

\bookmarksetup{startatroot}
\newrefcontext[sorting=none]
\printbibliography[
  heading=bibintoc,
  title={Publications during PhD Study},
  prenote=PubListPrenote,
  postnote=PubListPostnote
]
\end{refsection}

